Propagating leptons through matter with Muon Monte Carlo (MMC)

An accurate simulation of the propagation of muons through matter is needed for the analysis of data produced by muon/neutrino underground experiments. A muon may sustain hundreds of interactions before it is detected by the experiment. Since a small systematic uncertainty repeated hundreds of times may lead to sizable errors, requirements on the precision of the muon propagation code are very stringent. A new tool for propagating muon and tau charged leptons through matter that is believed to meet these requirements is presented here. An overview of the program is given and some results of its application are discussed.

==> allbib.tex <==
\bibitem{mythesis}
Chirkin, D.A., Cosmic Ray Energy Spectrum Measurement with the Antarctic Muon and Neutrino Detector Array (AMANDA), 2003, Ph.D. thesis, UC Berkeley

\bibitem{dcors_3}
Wiebel-Sooth, B. \& Biermann, P.L. 1999, Landolt-Bornstein, vol. VI/3c, Springer Verlag, p$37-90$

\bibitem{fermi}
Fermi, E. (1949), Phys. Rev. 75, 1169

\bibitem{bell}
Bell, A. R. (1978), Mon. Not. R. Astr. Soc. 182, 147 and 443

\bibitem{longair}
Longair, M. S. (1981) High Energy Astrophysics, Cambridge University Press

\bibitem{dcors_8}
Gaisser, T.K. 1990, Cosmic Rays and Particle Physics, Cambridge

\bibitem{gupta}
Gupta, M., \& Webber, W. R. (1989), Ap. J. 340, 1124

\bibitem{uchicago}
U. of Chicago, website: http://astroparticle.uchicago.edu

\bibitem{bmorse}
Morse, R., Neutrino Astronomy: First Light - Using the South Pole Ice Cap, Talk given at "Astrophysics from Antarctica" in Chicago, July 1997, AMANDA internal report 19980502

\bibitem{jjacobsen}
Jacobsen, J. E., Simulating the detection of muons and neutrinos in deep antarctic ice, 1996, Ph.D. thesis, U. of Wisconsin-Madison

\bibitem{dcors_1}
Gaisser, T.K., Halzen, F., \& Stanev, T. 1995, Phys. Rep. 258, 173

\bibitem{dcors_2}
Halzen, F., Proc. 26th ICRC (Salt Lake City, 1999)

\bibitem{AMANDA}
Andres, E., et al., AMANDA Collaboration, 22 Mar 2001, Nature 410, $441 - 443$

\bibitem{horandel}
H\"orandel, J., Astropart. Phys. 19 (2003) 193

\bibitem{solar}
http://www.ngdc.noaa.gov/stp/SOLAR/COSMIC\_RAYS/cosmic.html

\bibitem{SLC}
Chirkin, D., \& Rhode, W., 26th ICRC, HE.3.1.07, Salt Lake City, 1999

\bibitem{icrcHamburg}
Chirkin, D., \& Rhode, W., 27th ICRC, HE 220, Hamburg, 2001

\bibitem{hundertmark}
Hundertmark, S., DESY-PROC-1999-1, 276, 1999

\bibitem{wolfgang}
Rhode, W., \& C\^{a}rloganu, C., DESY-PROC-1999-01, 1999

\bibitem{workshopHamburg}
Chirkin, D., \& Rhode, W., Proceedings of 2nd Workshop on Methodical Aspects of Underwater/Underice Neutrino Telescopes, Hamburg, 2001

\bibitem{wiebusch}
Wiebusch, C., Muon Energy Reconstruction with AMANDA, AMANDA manuscript No 19990701, http://icecube.berkeley.edu/manuscripts/

\bibitem{ped}
Miocinovic, P., Muon Energy Reconstruction in the Antarctic Muon and Neutrino Detector Array (AMANDA), Ph.D. thesis, University of California, Berkeley, 2001

\bibitem{heiko}
Geenen, H., Energy reconstruction and spectral unfolding of atmospheric leptons with the AMANDA detector, diploma thesis, Wuppertal, 2002

\bibitem{dcors_5}
Heck, D., et al. 1998, Report FZKA 6019, Forschungszentrum Karlsruhe

\bibitem{tyce}
DeYoung, T. R., Observation of Atmospheric Muon Neutrinos with AMANDA, Dissertation, University of Wisconsin - Madison

\bibitem{dcors_4}
Knapp, J., Heck, D., \& Schatz, G. 1996, Report FZKA 5828, Forschungszentrum Karlsruhe

\bibitem{dcors_11}
Heck, D., Schr\"oder, F., et al., Proc. 26th ICRC (Salt Lake City, 1999)

\bibitem{corsika}
Heck, D., et al., CORSIKA: A Monte Carlo Code to Simulate Extensive Air Showers, physics manual distributed together with CORSIKA sources

\bibitem{dcors_6}
NSSDC: http://nssdc.gsfc.nasa.gov/space/model

\bibitem{dcors_7}
NGDC: http://www.ngdc.noaa.gov/seg/potfld/geomag.html, IGRF95 model

\bibitem{dcors_update}
dCORSIKA update report: http://icecube.wisc.edu/\~{ }dima/work/BKP/DCS/REPORT8/paper.ps.gz

\bibitem{dcors_9}
Volkova, L.V. 1980, Sov. J. Nucl. Phys. 31, 784 

\bibitem{dcors_mmc}
Muon Monte Carlo: a new high-precision tool for muon propagation through matter, ICRC 2001; updated results here: http://icecube.wisc.edu/\~{ }dima/work/

\bibitem{dcors_paolo}
suggested by Paolo Desiati, data provided by Buford Price (2002)

\bibitem{basiev}
Boziev, S. N., et al., 1989, INR preprint P-0630, Moscow

\bibitem{paolo}
Desiati, P., \& Rhode, W., 27th ICRC, HE 205 Hamburg, 2001

\bibitem{mmc}
mmc code homepage is http://icecube.wisc.edu/\~{ }dima/work/MUONPR/\\
mmc code available at http://icecube.wisc.edu/\~{ }dima/work/MUONPR/BKP/mmc.tgz

\bibitem{nure}
Numerical Recipes (W. H. Press, B. P. Flannery, S. A. Teukolsky, W. T. Vetterling), Cambridge University Press, 1988

\bibitem{symp}
Winterer, V.-H., SYMPHONY (talk presented at UC Berkeley, 1999),\\ available at http://www.rz.uni-freiburg.de/signatures/winterer\_vt/symphony/

\bibitem{mum}
Bugaev, E., Sokalski, I., \& Klimushin, S.,
MUM: Flexible precise Monte Carlo algorithm for muon propagation through thick layers of matter,
Phys. Rev. D 64, 074015 (2001), hep-ph/0010322, hep-ph/0010323, 2000

\bibitem{frank}
Schr\"{o}der, F., Rhode, W., \& Meyer, H., 27th ICRC, HE 2.2 Hamburg, 2001

\bibitem{dcors_10}
Daum, K., et al., Frejus Coll. 1995, Z. Phys. C 66, 417
Determination of the atmospheric neutrino spectra with the Frejus detector

\bibitem{pdb}
Hagiwara, K., et al., Particle Data Group, The European Physics Journal C vol. 15, pp 163-173, 2000

\bibitem{rossi}
Rossi, B., High Energy Particles, Prentice-Hall, Inc., Englewood Cliffs, NJ, 1952

\bibitem{kelner95}
Kelner, S.R., Kokoulin, R.P., \&
Petrukhin, A.A., About Cross Section for High Energy Muon Bremsstrahlung,
Preprint of Moscow Engineering Physics Inst., Moscow, 1995, no~024-95

\bibitem{heitler}
Bethe, H., \& Heitler, W, Proc. Roy. Soc., A146, 83 (1934)

\bibitem{bethe}
Bethe, H., Proc. Cambr. Phil. Soc., 30, 524 (1934)

\bibitem{kelner96}
Kelner, S.R., Kokoulin, R.P., \&
Petrukhin, A.A., Bremsstrahlung from Muons Scattered by Atomic Electrons, Physics
of Atomic Nuclei, Vol 60, No 4, 1997, 576-583

\bibitem{bugaev}
Bezrukov L.B., \& Bugaev, E.V., Nucleon shadowing effects in
photonuclear interactions, Sov. J. Nucl. Phys. 33(5), May 1981

\bibitem{kokgs}
Kokoulin, R.P., Nucl. Phys. B (Proc. Suppl.) 70
(1999) 475-479

\bibitem{rhode}
Rhode, W., Diss. Univ. Wuppertal, WUB-DIS- 93-11 (1993); W.
Rhode, Nucl. Phys. B. (Proc. Suppl.) 35 (1994), $250-253$

\bibitem{zeus}
Derrick, M., et al., ZEUS Collaboration, Z. Phys. C, 63 (1994) 391

\bibitem{pair1}
Kelner, S.R., \& Kotov, Yu.D., Muon energy loss
to pair production, Soviet Journal of Nuclear Physics, Vol 7, No 2, 237,
(1968)

\bibitem{pair2}
Kokoulin, R.P., \& Petrukhin, A.A., Analysis of the
cross section of direct pair production by fast muons, Proc. 11th Int. Conf.
on Cosmic Ray, Budapest 1969

\bibitem{pair}
Kokoulin, R.P., \& Petrukhin, A.A., Influence of the nuclear form
factor on the cross section of electron pair production by high energy
muons, Proc. 12th Int. Conf. on Cosmic Rays, Hobart 6 (1971), A 2436

\bibitem{mupair}
Kelner, S., Kokoulin, R., \& Petrukhin, A., Direct Production of Muon Pairs by High-Energy Muons,
Phys. of Atomic Nuclei, Vol. 63, No 9 (2000) 1603

\bibitem{scat}
Butkevitch, A., Kokoulin, R., Matushko, G., \& Mikheyev, S.,
Comments on multiple scattering of high-energy muons in thick layers, hep-ph/0108016, 2001

\bibitem{klein}
Klein, S., Suppression of bremsstrahlung and pair production due to environmental factors,
Rev. Mod. Phys., Vol 71, No 5 (1999) 1501

\bibitem{migdal}
Migdal, A., Bremsstrahlung and Pair Production in Condensed Media at High Energies
Phys. Rev., Vol. 103, No 6 (1956) 1856

\bibitem{polityko}
Polityko, S., Takahashi, N., Kato, M., Yamada, Y., \& Misaki, A.,
Muon cross-section with both the LPM effect and the Ter-Mikaelyan effect
at extremely high energies, Journal of Physics G: 2002 v.28, C.427-449,
hep-ph/9911330

\bibitem{polityko2}
Polityko, S., Takahashi, N., Kato, M., Yamada, Y., \& Misaki, A.,
The bremsstralung of muons at extremely high energies with LPM and
dielectric supression effect, Nuclear Instruments and Method in
Physics Research 2001 B 173, C.30-36

\bibitem{stanev}
Stanev, T., Vankov, Ch., Streitmatter, R., Ellsworth, R., \& Bowen, T.,
Development of ultrahigh-energy electromagnetic cascades in water and lead including the Landau-Pomeranchuk-Migdal effect
Phys. Rev. D 25 (1982) 1291

\bibitem{ternovskii}
Ternovskii, F., Effect of multiple scattering on pair production by high-energy particles in a medium,
Sov. Phys. JETP, Vol 37(10), No 4 (1960) 718

\bibitem{allm}
Abramowicz, H., Levin, E., Levy, A., \& Maor, U., A parametrization of $\sigma_T(\gamma^*p)$ above the resonance region for $Q^2\ge0$,
Phys. Lett. B269 (1991) 465

\bibitem{allm2}
Abramowicz, H., \& Levy, A., The ALLM parametrization of $\sigma_{tot}(\gamma^*p)$ an update,
hep-ph/9712415, 1997

\bibitem{dutta}
Dutta, S., Reno, M., Sarcevic, I., \& Seckel, D., Propagation of Muons and Taus at High Energies,
Phys. Rev. D 63 (2001) 094020, hep-ph/0012350

\bibitem{badelek}
Badelek, B., \& Kwiencinski, J., The low-$Q^2$, low-x region in electroproduction,
Rev. Mod. Phys. Vol 68 No 2 (1996) 445

\bibitem{whitlow}
Whitlow, L., Rock, S., Bodek, A., Dasu, S., \& Riordan, E., A precise extraction of $R=\sigma_L/\sigma_T$ from a global analysis of the SLAC deep
inelastic e-p and e-d scattering cross sections,
Phys. Lett. B250 No1,2 (1990) 193

\bibitem{badelek2}
Badelek, B., Kwiecinski, J., \& Stasto, A., A model for $F_L$ and $R=F_L/F_T$ at low x and low $Q^2$,
Z. Phys. C 74 (1997) 297

\bibitem{bouchta}
Bouchta, A., Muon Analysis with the AMANDA-B Four-String Detector, Ph.D. thesis, Stockholm University, 1998

\bibitem{Askebjer}
Askebjer, P., et al., Optical properties of the South Pole ice at depths between 0.8 and 1 kilometer, Science 267 (1995) 1147

\bibitem{pandel}
Pandel, D., Bestimmung von Wasser- und Detectorparametern und Reconstruction von Muonen bis 100 TeV mit dem Baikal-Neutrinoteleskop NT-72, diploma thesis, 1996

\bibitem{ptd}
Hundertmark, S., Vertical Ice Properties for the AMANDA-Simulation, AMANDA internal report No 20001001, also see http://icecube.wisc.edu/\~{ }karle/ptd/

\bibitem{cherenkov}
Jelly, J. V., Cerenkov Radiation and its Applications, Pergamon Press, New York, 1958

\bibitem{volkovaZ}
Volkova, L. V., Lebedev Physical Institute Report No. 72, 1969

\bibitem{bugaevF}
Bugaev, E. V., et al., Atmospheric Muon Flux at Sea Level, Underground and Underwater, hep-ph/9803488, also Phys. Rev. D58, 05401 (1998)

\bibitem{radlog}
Kelner, S., Kokoulin, R., \& Petrukhin, A., Radiation Logarithm in the Hartree-Fock Model,
Phys. of Atomic Nuclei, Vol. 62, No. 11, (1999) 1894

\bibitem{allm3}
Abramowicz, H., private communication (2001)

\bibitem{bugaev_shlepin}
Bugaev, E.V. \& Shlepin, Yu.V., Photonuclear interaction of high energy muons and tau-leptons,
Phys. Rev. D67 (2003) 034027, hep-ph/0203096

\bibitem{bugaev_montaruli}
Bugaev, E., Montaruli, T., Shlepin, Yu., \& Sokalski, I., Propagation of Tau Neutrinos and Tau Leptons through the Earth and their Detection in Underwater/Ice Neutrino Telescopes,
hep-ph/0312295

\bibitem{butmikh}
Butkevich, A.V. \& Mikheyev, S.P., Cross Section of the Muon-Nuclear Inelastic Interaction,
JETP, Vol 95, No 1 (2002) 11, hep-ph/0109060

\bibitem{butmikh2}
Butkevich, A.V. \& Mikheyev, S.P., Cross Section of Muon Photo-Nuclear Interaction,
28th ICRC, Tsukuba, 2003

\bibitem{ckmt}
Capella A., et at., 1994, Phys. Lett. B337, 358

\bibitem{abb}
Andreyev, Yu.M., Bezrukov, L.B., \& Bugaev, E.V., Phys. At. Nucl. 57, 2066 (1994)

\bibitem{abb2}
Bezrukov, L.B. \& Bugaev, E.V., 17th ICRC, Paris, 1981, Vol. 7, p. 102

\bibitem{my03icrc}
Chirkin, D.A., et al., Cosmic Ray Flux Measurement with AMANDA-II, 28th ICRC, Tsukuba, 2003

\bibitem{tables}
Groom, D.E., Mokhov, N.V., Striganov, S.I., Muon Stopping Power and Range Tables 10 MeV $-$ 100 TeV,
Atomic Data and Nuclear Data Tables, Vol. 78, 2, July 2001, 183,
http://pdg.lbl.gov/AtomicNuclearProperties/

\bibitem{ephys}
The European Physical Journal C, Review of Particle Physics, Vol. 15, 1-4, 2000

\bibitem{cern85}
Lohmann, W., Kopp, R., Voss, R., Energy Loss of Muons in the Energy Range 1-10000 GeV,
CERN 85-03, Experimental Physics Division, 21 March 1985

\bibitem{music}
Antonioli, P., Ghetti, C., Korolkova, E.V., Kudryavstsev, V.A., Sartorelli, G.,
Astropart. Phys. 7 (1997) 357

\bibitem{propmu}
Lipari, P., Astropart. Phys., 1 (1993) 195

\bibitem{lip}
Lipari, P., Stanev, T., Phys. Rev. D, Vol. 44, p. 3543, 1991

\bibitem{ps-brems}
Petrukhin, A.A. \& Shestakov, V.V.,
Can. J. Phys. 46, S377, 1968

\bibitem{tsai}
Tsai, Y.S., Rev. Mod. Phys. 46, 815, 1974

\bibitem{davies}
Davies, H., Bethe, H.A., \& Maximon, L.C., Phys. Rev. 93, 788, 1954

\bibitem{fluxes}
Chirkin, D., Fluxes of atmopheric leptons at 600 GeV - 60 TeV, hep-ph/0407078

\bibitem{ghill}
Hill, G.C., Detecting Neutrinos from AGN: New Fluxes and Cross Sections, astro-ph/9607140

\bibitem{ghill-thesis}
Hill, G.C., Experimental and Theoretical Aspects of High Energy Neutrino Astrophysics, Ph.D. thesis, University of Adelaide, 1996

\bibitem{anis}
Kowalski, M. \& Gazizov, A., High Energy Neutrino Generator for Neutrino Telescopes, 28th ICRC, Tsukuba, 2003

\bibitem{gandhi}
Gandhi, R., et al., Phys. Rev. D 58, 093009, 1998

\bibitem{gandhi96}
Gandhi, R., et al., Astropat. Phys. 5, 81, 1996

\bibitem{cteq6}
Pumplin, J., et al., New Generation of Parton Distributions with Uncertainties from Global QCD Analysis, hep-ph/0201195,
http://www.phys.psu.edu/~cteq/

\bibitem{earth}
Dziewonski, A., Earth Structure, Global, The Encyclopedia of Solid Earth Geophysics, James D.E.,
cd. (Van Nostrand Reinhold, New York, 1989) p.331

\bibitem{juliet}
Yoshida, S., Ishibashi, R., \& Miyamoto, H., Propagation of extremely high energy leptons in Earth, Phys. Rev. D 69, 103004, 2004

\bibitem{icecube}
http://www.icecube.wisc.edu/

\bibitem{monopole}
Ahlen, S.P., Theoretical and experimental aspects of the energy loss of relativistic heavily ionizing particles,
Rev. Mod. Phys., Vol 52, No 1 (1980) 121

\bibitem{monopole2}
Wick, S.D., Kephart, T.W., Weiler, T.J., Biermann, P.L., Signatures for a Cosmic Flux of Magnetic Monopoles, astro-ph/0001233

\bibitem{mustafa}
Mustafa, A.A.M., \& Jackson, D.F., Small-angle multiple scattering and spacial resolution in charged particle tomography,
Phys. Med. Biol., Vol 26 No 3 (1981) 461

\bibitem{lynch}
Lynch, G.R., Dahl, O.I., Approximations to multiple Coulomb scattering,
Nuclear Instruments and Method in Physics Research B 58 (1991) 6

\bibitem{smirnov_1}
Smirnov, G.I., On the universality of the x and a- dependence of the emc effect and its relation to parton distributions in nuclei,
Phys. Lett. B364 (1995) 87-92

\bibitem{smirnov_2}
Smirnov, G.I., Determination of the pattern of nuclear binding from the data on the lepton, Eur. Phys. J. C 10 (1999) 239


==> ltex <==
#!/bin/sh

if test "$1" = ""; then nice $0 muon; exit; fi

cat muon.tex | sed ':l1; s-^\(.*[^@]\)\(\\cite{[^}]*}\)\([^@]\)-\1@\2@\
\3-; t l1' | sed -n 's-.*\\cite{\([^}]*\)}.*-\1-gp' | sed 's-,-\
-g'  | awk 'BEGIN {n=0} {if($1 in a) print "repeated value" > "/dev/stderr"; else { b[n]=$1; n++; } a[$1]++} END {for(i=0;i<n;i++) print b[i]}' > aa
cat allbib.tex | grep -v '^ *%' > aa.tex
echo '\begin{thebibliography}{99}' > bib.tex
for i in `cat aa`; do cat aa.tex | sed -n '/^.bibitem{'$i'}/,/^ *$/p'; done >> bib.tex
echo '\end{thebibliography}' >> bib.tex
rm aa aa.tex

(echo latex $1.tex; latex $1.tex) &&
(echo latex $1.tex; latex $1.tex) &&
(echo latex $1.tex; latex $1.tex) &&
(echo dvips $1.dvi -o $1.ps; dvips $1.dvi -o $1.ps) &&
(echo rm $1.ps.gz; rm $1.ps.gz)
#(echo ps2pdf $1.ps; ps2pdf $1.ps) &&
(echo gzip $1.ps; gzip $1.ps) &&
(rm {*,*/*}.{aux,log,dvi,aix,idx,lo*,toc,*~})
#(echo gv $1.ps.gz; gv $1.ps.gz)


